Optimal Scoring Rules for Multi-dimensional Effort

This paper develops a framework for the design of scoring rules to optimally incentivize an agent to exert a multi-dimensional effort. This framework is a generalization to strategic agents of the classical knapsack problem (cf. Briest, Krysta, and V\"ocking, 2005, Singer, 2010) and it is foundational to applying algorithmic mechanism design to the classroom. The paper identifies two simple families of scoring rules that guarantee constant approximations to the optimal scoring rule. The truncated separate scoring rule is the sum of single dimensional scoring rules that is truncated to the bounded range of feasible scores. The threshold scoring rule gives the maximum score if reports exceed a threshold and zero otherwise. Approximate optimality of one or the other of these rules is similar to the bundling or selling separately result of Babaioff, Immorlica, Lucier, and Weinberg (2014). Finally, we show that the approximate optimality of the best of those two simple scoring rules is robust when the agent's choice of effort is made sequentially.

==> dynamic.tex <==
\section{Dynamic Effort}
\label{sec:dynamic}

\subsection{Dynamic Effort Model}
In the Dynamic Effort model, the agent makes the effort choice on tasks sequentially. 
In this paper, we focus on the setting where the order on the sequence of the tasks is fixed as exogenous, 
and the outcome of each task is publicly observed immediately 
after the agent reports the received signal to the principal. 
On each day $i$, let $\history_i$ be the sequence of reported signals and observed outcomes from day $1$ to day $i$, 
and $\privatehistory_i$ be the sequence of private signals the agent received from day $1$ to day~$i$. 
Since the private history is payoff irrelevant for the agent's expected future utility, 
it is without loss to focus on the strategies of the agent that only depend on the public history. 
By slightly overloading the notation, 
for any $i\in[n]$,
let $\strategy(\history_{i-1})\in\{0,1\}$ be the agent's effort choice at day $i$ given history $\history_{i-1}$
and $\strategy(\history_{i-1},\signal_i)\in\signals$ be the agent's reported signal at day $i$ given history $\history_{i-1}$.
We will focus on mechanisms that are incentive compatible on equilibrium path (\cref{def:dynamic IC}).

The timeline of our model is shown as follows.
\begin{enumerate}
\item The principal commits to an on-path incentive compatible mechanism with scoring rule
$\score(\history_n)\in [0,1]$
and a recommended strategy $\strategy$.
\item On each day $i\leq n$, the agent chooses effort $\effort_i=\strategy(\history_{i-1})$ 
and pays cost $\cost_i$.
Then outcome $\outcome_i$ is realized, 
and the agent receives the signals $\signal\in\signals$.
The agent reports $\strategy(\history_{i-1},\signal_i)$.
\item The agent receives reward $\score(\history_n)$.
\end{enumerate}

Let $\expecto[\strategy]{\cdot}$ be the expectation when the agent follows strategy $\strategy$ for all future tasks. 
\begin{definition}\label{def:dynamic IC}
A mechanism with scoring rule $\score$
and recommended strategy $\strategy$
is \emph{on-path incentive compatible}
if for any day $i$ such that the agent has followed strategy $\tau$ for all past days, 
\begin{align*}
\expecto[\strategy]{\score(\history_n) - \sum_{i\leq i' \leq n} \cost_{i'} a_{i'} \given \history_{i-1}}
\geq \expecto[\strategy']{\score(\history_n) - \sum_{i\leq i' \leq n} \cost_{i'} a_{i'} \given \history_{i-1}}.
\end{align*}
\end{definition}

% \begin{definition}\label{def:dynamic separate cap}
% A scoring rule $\score$ is a \emph{dynamic separate scoring rules with score cap} $B\geq 0$
% if there exists single-dimensional scoring rules $\score_1,\dots,\score_n$ and shifting parameter $d\geq 0$
% such that 
% $\score(\signal,\outcome) = \project_{[0,B]}\cbr{-d+\sum_{i\in[n]} \score_i(\signal_i,\outcome_i)}$.
% \end{definition}

==> symmetric.tex <==
\subsection{Symmetric Environments}
First, we consider the symmetric case where $n$ assignments have the same revealing probability $p$, cost $c$, and value $v$. 
\begin{theorem}\label{thm:symmetric-approx}
For $n$ i.i.d.\ assignments with the same revealing probability $p$, cost $c$, and value $v$, 
the maximum of the threshold scoring rule with threshold $1$ and a separate scoring rule with cap $1$ achieves an $\apxiid$-approximation to the optimal. The parameters of this separate scoring rule with score cap $1$ can be computed in polynomial time. 
% there exists a threshold scoring rule with parameter $k$,
% which requires the agent to choose a set $\effortset \subseteq [n]$ with $|\effortset|=k$
% and provides a reward of $1$
% if and only if the agent predicts all states correctly in $\effortset$,
% that is a constant approximation to the optimal scoring rule.
\end{theorem}


\begin{lemma}\label{lem:small c}
For any profile of values $\{\val_i\}_{i=1}^n$ and costs $\{\cost_i\}_{i=1}^n$, 
if $\cost_i\leq\frac{p}{96}$ for all $i\in[n]$,
there exists a separate scoring rule with score cap $1$ that is a $48$-approximation to the optimal. The parameters of this separate scoring rule with score cap $1$ can be computed in polynomial time.  
\end{lemma}
\begin{proof}
Let $\effortset$ be the set of tasks that are added greedily according to the ratio $\frac{\val_i}{\cost_i}$ until exceeding $\frac{1}{48}$.
By \cref{thm:budget inflation}, 
there exists a polynomial time algorithm for computing an incentive compatible mechanism 
using a separate scoring rule with score cap $1$ 
that incentives the agent to exert effort for all tasks in $\effortset$.
Moreover, $\sum_{i\in\effortset} \val_i$ is at least the optimal fractional knapsack value given budget $\frac{1}{48}$, 
where the latter is a $48$-approximation to the optimal utility of the principal given budget $1$.
\end{proof}






\begin{lemma}\label{lem:symmetric opt}
For $n$ i.i.d.\ assignments with the same revealing probability $p$, cost $c$, and value $v$, 
there exists an optimal proper scoring rule which assigns reward $\score(\signal,\outcome) = s_k$ if and only if the agent reports exactly $k$ informative signals, i.e. $|\{i:\sigma_i \neq \bot\}| = k$. 
This optimal scoring rule satisfies $s_{k+1}\geq s_k \geq \frac{s_{k+1}}{2}$
for all $1 \leq k \leq n-1$.
% $n$ rewards $s_{k}$ for all $k \in [n]$
% such that the agent chooses a subset $\effortset \subseteq [n]$
% and receives reward $s_k \in [0,1]$ where $k = |\effortset|$ be the size of $\effortset$
% if and only if the agent predicts all outcomes correctly in $\effortset$.
\end{lemma}

\begin{proof}
We show that any effort level incentivized by a proper scoring rule $\score$ can be incentivized by a scoring rule $\score'$ that assigns reward $s_k$ for $k$ informative signals. 

Since the outcomes of assignments are i.i.d.\ , without loss of generality, suppose the agent only exerts effort on the first $\neffort$ assignments $\effortset=\{1,\dots, \neffort\}$ for scoring rule $\score$. The expected score by exerting effort on $\effortset$ is $\expect[\effortset]{\expect[\signal]{\score(\signal,\outcome)}}$. For the assignments on which the agent exerts no effort, the posterior beliefs on these assignments do not change. Thus, $\expect[\effortset]{\expect[\signal]{\score(\signal,\outcome)}}$ does not depend on the posterior beliefs of the assignments $i>\neffort$. 

For each $k \in [l]$, let $s_k$ be the expected score of $\score$ over all posteriors with exactly $k$ informative signals. Then, the scoring rule $\score'$ with score $s_k$ for $k$ informative signals achieves the same expected score given by $\score$ if the agent exerts effort on any set $\effortset' \subseteq \effortset$. Since $\effortset$ is incentive compatible for $\score$, this set $\effortset$ is also incentive compatible for $\score'$.
%This expected score function $\hat{\score}$ can be implemented by such a scoring rule with rewards $r_i=\hat{\score}(i)$ for all $i \in [l]$.
%Let the number of assignments that the agent receives the informative signals be $\knowthetruth$. Then, the score with $k$ informative signals is $S(\knowthetruth)$. This expected score function $\hat{\score}$ can be implemented by such a scoring rule with rewards $r_i=\hat{\score}(i)$ for all $i \in [l]$.
%Therefore, the expected score $\tilde{S}$ can be written as a function of the number of assignments that the agent knows the truth. Let the number of assignments that the agent receives the informative signals be $\knowthetruth$. Then, the score with $k$ informative signals is $S(\knowthetruth)$. This expected utility function $u$ can be implemented such a scoring rule with rewards $r_i=S(i)$ for all $i \in [N]$.

By incentive compatibility, the rewards $s_k$ is weakly increasing in $\knowthetruth$, for $0 \leq \knowthetruth \leq \neffort$. Since the agent can guess the outcome of each assignment with probability $\sfrac{1}{2}$, we have that $s_k \geq \sfrac{s_{k+1}}{2}$, which completes the proof. 
% By the symmetry of assignments, $\hat{\util}$ does not depend on the no-effort assignments $\posterior_i, i>\neffort$, and can be written as a function of the number of assignments that the agent knows the truth. Let the number of assignments that the agent has belief $0$ or $1$ be $\knowthetruth$, the utility be $\util(\knowthetruth)$. By incentive compatibility, $\util$ is weakly increasing in $\knowthetruth$, with $\knowthetruth$ taking value in $[\neffort]$. We also know that $\util(\knowthetruth)\geq \sfrac{1}{2}\cdot\util(\knowthetruth+1)$, since the agent can guess the correct answer with probability $\sfrac{1}{2}$.
\end{proof}



\begin{lemma}\label{lem:symmetric-eps-small}
For $n$ i.i.d.\ assignments with $p \leq 1/2$ and $\epsilon = \frac{p}{2c} -1 \in (0,1/8)$, the maximum effort level that can be incentivized by a scoring rule is at most $-4 \frac{\log(\epsilon+1)}{\log(1-p)}$.
\end{lemma}

\begin{proof}
We show that the incentive compatibility constraint is not feasible for the effort level $-4\frac{\log(\epsilon+1)}{\log(1-p)}+1$ in the optimal scoring rule $\score$. By Lemma~\ref{lem:monotone task}, all effort levels greater than $-4 \frac{\log(\epsilon+1)}{\log(1-p)}$ can not be incentivized. 

The agent chooses to exert effort on $l+1$ assignments if and only if the expected utility of effort level $l+1$ is at least the expected utility of effort level $l$. By Lemma~\ref{lem:symmetric opt}, the optimal scoring rule assigns reward $s_k$ for $k$ informative signals. Since $n$ i.i.d. assignments have the same revealing probability $p$, the number of informative signals $k$ is from a binomial distribution $\binomial(\neffort,p)$ if the agent exerts effort on $\neffort$ assignments. The optimal scoring rule must satisfy the following incentive compatibility constraint
$$
\expect[\knowthetruth\sim\binomial(\neffort+1, p)]{\reward_\knowthetruth}-(\neffort+1)\cost \geq
\expect[\knowthetruth\sim\binomial(\neffort, p)]{\reward_\knowthetruth}-\neffort\cost.
$$
Then, we show that this incentive compatibility constraint is not satisfied when $l = -4 \frac{\log(\epsilon+1)}{\log(1-p)}$. Let $X_{\neffort,p}$ be a random variable from the binomial distribution $\binomial(\neffort, p)$. Let $f(k, \neffort, p) = \prob{X_{\neffort,p} = k}$ be the probability that $X_{\neffort,p}$ takes value $k$.  The difference between the expected utilities of effort levels $l+1$ and $l$ is 
\begin{align}\label{eqn:ic}
&\expect[\knowthetruth\sim\binomial(\neffort+1, p)]{\reward_\knowthetruth} - \expect[\knowthetruth\sim\binomial(\neffort, p)]{\reward_\knowthetruth} - \cost \nonumber\\
&= p \sum_{k=0}^{l} f(k,l,p) \reward_{\knowthetruth+1} + (1-p)\sum_{k=0}^{l} f(k,l,p) \reward_{\knowthetruth} - \sum_{k=0}^{l} f(k,l,p) \reward_{\knowthetruth} - \cost \nonumber\\
&=p \sum_{k=0}^{l} f(k,l,p) (\reward_{\knowthetruth+1} - \reward_{\knowthetruth}) - \cost.
\end{align}

We now show the right hand side in equation~(\ref{eqn:ic}) is strictly negative when the effort level $l = -4 \frac{\log(\epsilon+1)}{\log(1-p)}$. Recall $\epsilon = \sfrac{p}{2c}-1$. Since $-\log(1-p) \geq p$ and $\log(1+\epsilon) \leq \epsilon$, we have $\neffort \leq \sfrac{4\epsilon}{p}$. The mean of the Binomial distribution $\binomial(\neffort, p)$ is 
$$
lp \leq \frac{4\epsilon}{p} \cdot p =  4\epsilon \leq 1/2.
$$ 
The probability mass function $f(k,l,p)$ of the Binomial distribution $\binomial(\neffort, p)$ is monotone decreasing for $k > \neffort p$. Sicne $p\leq 1/2$ and $\neffort p \leq 1/2$, we have 
$$
f(0,\neffort,p) = (1-p)^\neffort = \frac{1-p}{\neffort p} \cdot f(1,\neffort,p) \geq f(1,\neffort,p).  
$$
Therefore, the probabilities $f(k,l,p)$ are non-increasing with respect to $k$. By Lemma~\ref{lem:symmetric opt}, the rewards of the optimal scoring rule satisfies $\reward_{k+1} \geq \reward_{k} \geq \reward_{k+1}/2$ for all $1\leq k \leq n$. For any $k \leq n$,  we have $\reward_0 \geq 2^{-k}\reward_k$, which implies $s_k-s_0 \leq (1-2^{-k})s_k \leq (1-2^{-k})$. If we consider $s_{k+1}-s_k$ in the right side of (\ref{eqn:ic}) as the weight on probability $f(k,\neffort,p)$, then these weights should satisfy the constraints $\sum_{i=0}^k (s_{i+1}-s_i) \leq (1-2^{-(k+1)})$ for $0 \leq k \leq \neffort$. Since the probabilities $f(k,l,p)$ are non-increasing, the first term in the right side of (\ref{eqn:ic}) is maximized by moving the weights to small $k$ terms under the constraints. By taking $\reward_{k+1}-\reward_k = 2^{-(k+1)}$ for all $k$, the first term in the utility difference is upper bounded by
\begin{align*}
p\sum_{k=0}^{l} f(k,l,p)2^{-(k+1)} = \frac{p}{2} \Big(1-\frac{p}{2}\Big)^l\sum_{k=0}^{l} f(k,l,\sfrac{p}{2-p}) = \frac{p}{2} \Big(1-\frac{p}{2}\Big)^l.
\end{align*}
Since $l = -4 \frac{\log(\epsilon+1)}{\log(1-p)} \geq \frac{2}{p}\log(1+\epsilon)$ for $p\leq \sfrac{1}{2}$ and $\epsilon = \frac{p}{2c}-1$, we have
\begin{align*}
\frac{p}{2} \Big(1-\frac{p}{2}\Big)^l - \cost \leq p\Big[\frac{1}{2} \Big(1-\frac{p}{2}\Big)^{\frac{2}{p}\cdot \log(1+\epsilon)}-\frac{c}{p}\Big] < p\Big(\frac{1}{2} \frac{1}{1+\epsilon} - \frac{c}{p}\Big) = 0.
\end{align*}
Hence, the incentive compatibility constraint is not satisfied for the effort level $l = -4 \frac{\log(\epsilon+1)}{\log(1-p)}$.

\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:symmetric-approx}]
We consider the following two cases based on the ratio of $c$ and $p$: (1) $\sfrac{p}{c} \geq 96$; (2) $\sfrac{p}{c} < 96$. For the first case $\sfrac{p}{c} \geq 96$, by Lemma~\ref{lem:small c}, we find a separate scoring rule with cap $1$ to achieve a $48$-approximation. We then focus on the second case where $\sfrac{p}{c} < 96$. Let $\epsilon = \sfrac{p}{2c}-1$. If $\epsilon\leq 0$, by \Cref{lem:single opt} and  \Cref{lem:monotone task}, the optimal level of effort is $0$.

For the case where $\epsilon \in (0,47)$, we show that the threshold scoring rule with threshold $k = 1$ achieves a $480$-approximation.

When the agent exerts effort on $\neffort$ assignments, the agent will get at least one informative signal with the probability $1-(1-p)^{\neffort}$. In this case, the threshold scoring rule assigns score $1$ to the agent. Otherwise, the agent gets no informative signal and guesses the outcome for one assignment with expected score $1/2$. Thus, the total expected utility for exerting effort on $\neffort$ assignments is 
$$
1-(1-p)^{\neffort}+\sfrac{1}{2}(1-p)^{\neffort} - \neffort\cost.
$$
% will be the expected score $[1-(1-p)^{\neffort}+\sfrac{1}{2}(1-p)^{\neffort}]$ minus the total cost $\neffort\cdot\cost$.

The marginal gain in the expected score for exerting effort on $\neffort+1$ assignments is
\begin{align}
    [1-(1-p)^{\neffort+1}+\sfrac{1}{2}(1-p)^{\neffort+1}]-[1-(1-p)^{\neffort}+\sfrac{1}{2}(1-p)^{\neffort}]=\sfrac{1}{2}\cdot p(1-p)^\neffort
\end{align}

The marginal gain is monotone decreasing in the amount of effort $\neffort$. The agent will exert effort until $\sfrac{1}{2}\cdot p(1-p)^\neffort>\cost$, which implies $l\geq \min\{\lceil -\frac{\log(\epsilon+1)}{\log(1-p)}\rceil, n\}$, where $\epsilon+1=\frac{p}{2\cost}$. The optimal amount of effort will be at least $1$. 
When $n < \lceil -\frac{\log(\epsilon+1)}{\log(1-p)}\rceil$, the threshold scoring rule is optimal since all $n$ assignments are incentivized by the threshold scoring rule. 
When $n \geq \lceil -\frac{\log(\epsilon+1)}{\log(1-p)}\rceil$, we analyze the threshold scoring rule in the following four cases. 

For $\epsilon\in(0, 1/8), p\leq 1/2$, by \Cref{lem:symmetric-eps-small}, the optimal level of effort is at most $4\neffort$, which implies this threshold scoring rule is a $4$-approximation.

For $\epsilon\in (0, 1/8), p> 1/2$, the optimal level of effort is $\opteffort\leq\frac{1}{c}\leq \frac{3}{p}\leq 6$. Since this threshold scoring rule incentivizes at least one assignment, this threshold scoring rule achieves a $6$-approximation.
    
For $\epsilon\in[1/8, 47), p\leq 1/2$, the level of effort incentivized by the threshold scoring rule is 
$$
\neffort \geq \lceil -\frac{\log(\epsilon+1)}{\log(1-p)}\rceil\geq \frac{\log(9/8)}{2p}\geq\frac{\log(9/8)}{2\cdot 96c}\geq \frac{1}{1700c}\geq \frac{\opteffort}{1700}.
$$ 
The approximation ratio is $1700$.
    
For $\epsilon\in [1/8, 47), p\geq 1/2$, the optimal level of effort is $\opteffort\leq\frac{1}{c}\leq \frac{96}{p}\leq 192$. The approximation ratio is at most $192$.
\end{proof}


% Since $\sum_{k=0}^l \reward_{\knowthetruth+1} - \reward_{\knowthetruth} = \reward_{l+1} - \reward_0\leq 1$, the first term in the utility difference is upper bounded by $p\prob{}{0;l,p} = p(1-p)^l$. For $l =  - \frac{\log(\epsilon+1)}{\log(1-p)}$, we have
% $$
% p(1-p)^l - \cost = p\Big(\frac{1}{1+\epsilon} - \frac{\cost}{p}\Big) = p\Big(\frac{2\cost}{p} - \frac{\cost}{p}\Big)
% $$



\begin{theorem}\label{thm:approx nonsymmetric cost}
For $n$ assignments with the same revealing probability $p$ and value $\val$, but different costs $\{\cost_i\}_{i\in [N]}$, there exists a polynomial time algorithm for computing an incentive compatible mechanism that is an $\apxratioc$-approximation to the optimal.
\end{theorem}

\begin{proof}
We divide the $n$ assignments into two sets $A_1,A_2$ based on the ratio $\sfrac{p}{\cost_i}$ as follows
$$
A_1 = \{i: \sfrac{p}{\cost_i} \geq 96\}; \qquad A_2 = \{i: \sfrac{p}{\cost_i} < 96\}.
$$
We show that, on each of the two sets $A_1, A_2$, we find a scoring rule achieves an $\apxc$-approximation to the optimal scoring rule on that set. By using the scoring rule on the set with a higher total value incentivized by the optimal scoring rule, the mechanism achieves a $\apxratioc$ approximation.



The following benchmark environment will be useful in the analysis:   the $n$ assignments, the same revealing probability $p$, and cost $c$ for any $c > \sfrac{p}{96}$. Let $\opt(\cost)$ be the number of assignments incentivized by the optimal scoring rule.  
Let $\obj(\cost)$ be the number of assignments that is incentivized by the threshold scoring rule with threshold $k=1$. 

By \Cref{lem:small c}, we compute a separate scoring rule with cap $1$ that achieves a $48$-approximation on the set $A_1$. It only remains to show there is a $\apxc$-approximation scoring rule on the set $A_2$. We use the threshold scoring rule with threshold $k=1$ on the set $A_2$ as in \Cref{thm:symmetric-approx}. 

We first lower bound the level of effort for the threshold scoring rule with threshold $k=1$. For the threshold scoring rule, the agent will start exerting effort on the set $A_2$ in increasing order of cost $\cost_i$. Therefore, we sort the assignments in the set $A_2$ in increasing order of cost: $\cost_1\leq \cost_2\leq \cdots\leq \cost_{n_2}$, where $n_2 = |A_2|$. Let $\neffort$ be the number of assignments incentivized by a threshold scoring rule with threshold $k=1$. Similar as Proof of \Cref{thm:symmetric-approx}, agent stops when cost of doing assignment $\neffort+1$ is less than the marginal gain on the expected score for doing one more assignment. Thus, we have
\begin{align*}
    \frac{p}{2}(1-p)^{\neffort}<\cost_{\neffort+1};
    \qquad
     \frac{p}{2}(1-p)^{\neffort-1}\geq \cost_{\neffort}.
\end{align*}
Since costs are sorted in increasing order, the threshold scoring rule with threshold $k=1$ can incentivize more assignments in non-symmetric case than that in the symmetric case with cost $\cost_{\neffort+1}$, i.e. $\neffort \geq \obj(\cost_{\neffort+1})$. 

We now upper bound the level of effort for the optimal scoring rule. Let $\effortset$ be the set of assignments incentivized by the optimal scoring rule on the set $A_2$. By the monotonicity in assignments in \Cref{lem:monotone task}, we have $\effortset' = \effortset \cap \{i: i\in A_2, \cost_i \geq \cost_{\neffort+1}\}$ can also be incentivized. By the monotonicity in cost in \Cref{lem:monotone-cost}, the set $\effortset'$ can still be incentivized if we change all costs in $\effortset'$ to $\cost_{\neffort+1}$, which implies that $\opt(\cost_{\neffort+1})\geq |\effortset'| \geq |\effortset|-\neffort$. 

By \Cref{thm:symmetric-approx}, we have $\apxiid\,\obj(\cost_{\neffort+1})\geq \opt(\cost_{\neffort+1})$. Thus, we have 
$$
\apxiid\, \neffort \geq \apxiid\, \obj(\cost_{\neffort+1}) \geq \opt(\cost_{\neffort+1}) \geq |\effortset| - \neffort, 
$$
which implies
$\apxc \neffort\geq |\effortset|$, i.e.\ the threshold scoring rule with threshold $k =  1$ is a $\apxc$-approximation on the set $A_2$.
\end{proof}


\begin{lemma}[Monotonicity in cost]~\label{lem:monotone-cost}
Fix the probability $p$ of receiving an informative signal. For any two set of costs $\{\cost_i\}_{i\in[N]}$
and $\{\cost'_i\}_{i\in[N]}$ such that  $\cost'_i\leq\cost_i$
for all $i\in [N]$. 
For any subset $\effortset\subseteq [N]$ of assignments, 
if there exists an incentive compatible mechanism with scoring rule $\score$  and recommendation set $\effortset\subseteq [N]$
 given $\{\cost_i\}_{i\in[N]}$, 
there also exists an incentive compatible mechanism with  scoring rule $\score'$ and recommendation set $\effortset$
given $\{\cost'_i\}_{i\in[N]}$.
\end{lemma}

\begin{proof}[Proof of \cref{lem:monotone-cost}]
Let the signal space be the product of signal space in the recommendation set and in the non-recommendation set, i.e.\  $\signal=\signal_{\effortset}\times\signal_{[N]\setminus \effortset}$. Truncate scoring rule $\score$ to the recommendation set $\effortset$ by setting score to a constant with regard to the signals in the non-recommendation set: $\score'(\signal, \outcome)=\score(\signal_{\effortset}\times \{\bot\}^{N-|\effortset|}, \outcome)$. Thus, the agent has no incentive to exert effort on the non-recommendation set $[N]\setminus\effortset$. For any set of effort $\effortset'$, consider the expected utility difference of exerting effort on $\effortset$ and $\effortset'$, which equals $\expect[\effortset]{\score}-\expect[\effortset']{\score}$. Decreasing the costs only makes this utility difference larger, which means $\effortset$ is incentive compatible with scoring rule $\score'$.
\end{proof}

\begin{lemma}\label{lem:asym-upper-bound}
For any set $\effortset$ such that $p\leq 1/2$ and $\cost_i \geq \sfrac{p}{2.1}$ for all task $i\in\effortset$, if the set $\effortset$ can be incentivized by a proper scoring rule, 
then $\abs{\effortset} \leq \frac{-3\log(p/2c^*)}{\log(1-p)} +1$, where $c^* = \max_{i \in \effortset} \cost_i$.
\end{lemma}
\begin{proof}
We first consider the  incentive compatibility constraint of the assignment in $\effortset$ with the highest cost. Let $i^* = \argmax_{i\in\effortset}\cost_i$. 
By the incentive compatibility constraint on assignment $i^*$, we have
$$
\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)}} - \expect[\effortset\backslash\{i^*\}]{\expect[\signal]{S(\signal,\outcome)}} - \cost_{i^*} \geq 0.
$$
Let $\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_{i^*} = \bot}$ be the expected score conditioned on signal $\signal_i = \bot$ when the agent exerts effort on $\effortset$. We have $\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_{i^*} = \bot} = \expect[\effortset\backslash\{i^*\}]{\expect[\signal]{S(\signal,\outcome)}}$. Similarly, let $\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_{i^*} \neq \bot}$ be the expected score conditioned on $\signal_{i^*} \neq \bot$ with effort set $\effortset$. Then, the incentive compatibility constraint on $i^*$ is
\begin{align}\label{eqn:asym_ic}
&p\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_{i^*} \neq \bot} + (1-p)\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_{i^*} = \bot} - \expect[\effortset\backslash\{i^*\}]{\expect[\signal]{S(\signal,\outcome)}} = \nonumber\\
&= p\bigg(\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_{i^*} \neq \bot} - \expect[\effortset\backslash\{i^*\}]{\expect[\signal]{S(\signal,\outcome)}}\bigg) \geq \cost_{i^*}.
\end{align}

We now show the upper bound on the difference between the expected score with signal $\signal_{i^*}\neq \bot$ and the expected score with signal $\signal_{i^*} = \bot$. For any $i\in\effortset$, let $\event_i$ be the event that at least one signal that is not $\bot$ from tasks $\effortset\backslash\{i\}$.  
Let $q$ be the probability that $\event_i$ happens
\begin{align*}
q=\prob[\effortset]{\event_i} = (1-(1-p)^{\abs{\effortset}-1}). 
\end{align*} 

We bound the expected score difference under the following two cases: (1) event $\event_{i^*}$ does not happen; (2) event $\event_{i^*}$ happens.
% Then, we have
% $$
% \expect[\effortset\backslash\{i^*\}]{\expect[\signal]{S(\signal,\outcome)}} = q\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \event} + (1-q)\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_i = \bot, \forall i \in \effortset}.
% $$

We first upper bound the expected score difference conditioned on event $\bar{\event}_{i^*}$. Since the agent can guess the outcome of assignment $i$ with probability $1/2$, we have
$$
\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_{i^*}= \bot, \bar{\event}_{i^*} } \geq \expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_{i^*}\neq \bot, \bar{\event}_{i^*} }/2,
$$
which implies the expected score difference conditioned on $\bar{\event}_{i^*}$ is at most $1/2$. 

We now upper bound the expected score difference conditioned on event $\event_{i^*}$. We show that $\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_{i^*} = \bot, \event_{i^*}} \geq 3/4$, which implies the expected score difference conditioned on $\event_{i^*}$ is at most $1/4$. For any assignment $i\neq i^*, i \in \effortset$, by the incentive compatibility constraint on assignment $i$, we have
$$
p\bigg(\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_i \neq \bot} - \expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_i = \bot}\bigg) \geq \cost_i.
$$
Since the scoring rule is proper, we have $\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_i \neq \bot} \geq \expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_i = \bot}/2$. Thus, the expected score conditioned on signal $\signal_i \neq \bot$ is at least
$$
\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_i \neq \bot} \geq \frac{2\cost_i}{p} \geq \frac{1}{1+\epsilon}.
$$
Let $\event_i$ be the event that there is at least one signal is not $\bot$ from $\effortset\backslash \{i\}$. We upper bound the expected score conditioned on signal $\signal_i \neq \bot$ by 
\begin{align*}
\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_i \neq \bot} =& (1-p)^{|\effortset|-1}\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_i \neq \bot, \bar{\event_i}} \\
&+ (1- (1-p)^{|\effortset|-1})\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_i \neq \bot, \event_i} \\
\leq & \expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_i \neq \bot, \bar{\event_i}} + (1- (1-p)^{|\effortset|-1}).
\end{align*}
By the monotonicity in cost in Lemma~\ref{lem:monotone-cost} and Lemma~\ref{lem:symmetric-eps-small}, we have $|\effortset| \leq -4\frac{\log(1+\epsilon)}{\log(1-p)}$. Thus, we have
\begin{align*}
\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_i \neq \bot, \bar{\event_i}} &\geq \expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_i \neq \bot} - (1- (1-p)^{|\effortset|-1}) \\
&\geq \frac{1}{1+\epsilon} - \bigg(1-\frac{1}{(1+\epsilon)^4}\bigg)\geq \frac{3}{4}.
\end{align*}
Since the scoring rule is proper, we have  $\expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_{i^*} = \bot, \event_{i^*}} \geq 3/4$, which implies the expected score difference conditioned on $\event_{i^*}$ is at most $1/4$. 

Combining the above two cases, the expected score difference in the equality~(\ref{eqn:asym_ic}) is
\begin{align*}
    \expect[\effortset]{\expect[\signal]{S(\signal,\outcome)} \mid \signal_{i^*} \neq \bot} - \expect[\effortset\backslash\{i^*\}]{\expect[\signal]{S(\signal,\outcome)}} 
    &\leq \prob{\event_{i^*}}\frac{1}{4} + \prob{\bar{\event}_{i^*}}\frac{1}{2} \\
    &\leq q/4 + (1-q)/2 = 1/2 -q/4.
\end{align*}
By the inequality (\ref{eqn:asym_ic}), we have 
$$
p\bigg(\frac{1}{2}-\frac{q}{4}\bigg) \geq \cost_{i^*}.
$$
Let $\epsilon^* = \sfrac{p}{2\cost_{i^*}}-1$. Then, the maximum cost $\cost_{i^*} = \frac{p}{2(\epsilon^*+1)}$, which implies 
$$
q \leq \frac{2\epsilon^*}{1+\epsilon^*} \leq 2\epsilon^*.
$$
Since $q = 1-(1-p)^{|\effortset|-1}$ and $-\log(1-2\epsilon^*) \leq 3\log(1+\epsilon^*)$ for $\epsilon^* \in (0,0.05)$, we obtain 
$$
|\effortset| \leq \frac{\log(1-2\epsilon^*)}{\log(1-p)} +1 \leq \frac{-3\log(1+\epsilon^*)}{\log(1-p)} +1,
$$
where $\epsilon^* = \sfrac{p}{2\cost_{i^*}}-1$.
\end{proof}

